Directly imaging damped Ly-alpha galaxies at z>2. II: Imaging and spectroscopic observations of 32 quasar fields

Damped Ly-alpha absorbers (DLAs) are a well-studied class of absorption line systems, and yet the properties of their host galaxies remain largely unknown. To investigate the origin of these systems, we have conducted an imaging survey of 32 quasar fields with intervening DLAs between z~1.9-3.8, leveraging a technique that allows us to image galaxies at any small angular separation from the background quasars. In this paper, we present the properties of the targeted DLA sample, new imaging observations of the quasar fields, and the analysis of new and archival spectra of the background quasars.

==> tab_mtl.tex <==
 
 
\begin{deluxetable}{lcccccccccccccccccc}
\rotate
\tablewidth{0pc}
\tablecaption{DLA METAL SUMMARY\label{tab:mtl}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{Quasar} &\colhead{RA (2000)} & \colhead{DEC (2000)} & \colhead{$z_{em}$} & \colhead{$z_{abs}$} & \colhead{log \nhi} & 
\colhead{f$_M^a$} & \colhead{[M/H]} &
\colhead{$\sigma(M)$} &
\colhead{f$_\alpha^b$} & \colhead{[$\alpha$/H]} &
\colhead{$\sigma(\alpha$)} &
\colhead{f$_{Zn}^c$} & \colhead{[Zn/H]} &
\colhead{$\sigma$(Zn)} &
\colhead{f$_{Fe}^d$} & \colhead{[Fe/H]} &
\colhead{$\sigma$(Fe)} & \colhead{Ref}}
\startdata
--2114--
J073149.50+285448&07:31:49.50&+28:54:48.6&3.676&2.6878&$20.60^{+0.10}_{-0.10}$& 1&$-1.45$&0.17& 1&$-1.45$&0.14& 3&$-1.16$&    & 1&$-1.46$&0.11&0\\
J095604.43+344415&09:56:04.43&+34:44:15.5&3.427&2.3887&$21.10^{+0.15}_{-0.15}$& 2&$-1.00$&&     2&$-1.48$&    & 1&$-1.00$&0.09& 1&$-1.46$&0.11&0\\
J234349.41-104742&23:43:49.41&-10:47:42.0&3.616&2.6880&$20.60^{+0.10}_{-0.10}$&13&$-1.27$&0.20&13&$-1.27$&0.20& 3&$-0.63$&    & 1&$-1.77$&0.03&0\\
J034300.88-062229&03:43:00.88&-06:22:29.9&3.623&2.5713&$20.75^{+0.20}_{-0.20}$&14&$-2.02$&0.26& 3&$-1.24$&    & 3&$-0.72$&    & 1&$-2.32$&0.05&0\\
J235152.80+160048&23:51:52.80&+16:00:48.9&4.694&3.7861&$20.85^{+0.10}_{-0.10}$&14&$-2.03$&0.20& 2&$-2.26$&    & 0&$     $&    & 1&$-2.33$&0.06&0\\
--0042--
J094927.88+111518&09:49:27.88&+11:15:18.2&3.824&2.7584&$20.85^{+0.10}_{-0.10}$& 1&$-0.95$&0.10& 1&$-0.95$&0.02& 0&$     $&    & 1&$-1.20$&0.05&0\\
J101806.28+310627&10:18:06.28&+31:06:27.2&3.629&2.4592&$20.35^{+0.10}_{-0.10}$&13&$-1.19$&0.28& 2&$-1.48$&    & 3&$-0.91$&    & 1&$-1.50$&0.03&0\\
J085143.72+233208&08:51:43.72&+23:32:08.9&4.490&3.5297&$21.10^{+0.10}_{-0.10}$& 2&$-1.05$&&     2&$-1.04$&    & 1&$-1.05$&0.11& 4&$-1.51$&0.05&0\\
J095605.09+144854&09:56:05.09&+14:48:54.7&3.400&2.6606&$20.85^{+0.10}_{-0.10}$& 1&$-1.46$&0.12& 1&$-1.46$&0.07& 1&$-1.17$&0.11& 1&$-1.63$&0.08&0\\
J115130.48+353625&11:51:30.48&+35:36:25.0&3.500&2.5978&$20.90^{+0.10}_{-0.10}$& 1&$-1.28$&0.11& 1&$-1.28$&0.05& 0&$     $&    & 1&$-1.74$&0.01&0\\
J212357.56-005350&21:23:57.56&-00:53:50.1&3.583&2.7803&$20.70^{+0.10}_{-0.10}$&13&$-1.59$&0.15&13&$-1.59$&0.15& 0&$     $&    & 1&$-1.88$&0.02&0\\
J040718.06-441014&04:07:18.06&-44:10:14.0&3.000&1.9127&$20.55^{+0.10}_{-0.10}$& 1&$-0.77$&0.11& 1&$-0.77$&0.05& 1&$-0.41$&0.09& 1&$-0.59$&0.03&0\\
J025518.58+004847&02:55:18.58&+00:48:47.6&3.996&3.2530&$20.60^{+0.10}_{-0.10}$& 1&$-0.80$&0.11& 1&$-0.80$&0.05& 3&$-0.68$&    & 1&$-1.28$&0.02&0\\
J081618.99+482328&08:16:18.99&+48:23:28.4&3.582&2.7066&$20.70^{+0.15}_{-0.15}$& 1&$-2.36$&0.15& 1&$-2.36$&0.02& 3&$-1.17$&    & 1&$-2.41$&0.03&0\\
J090810.36+023818&09:08:10.36&+02:38:18.7&3.710&2.9586&$21.10^{+0.10}_{-0.10}$& 1&$-0.93$&0.12& 1&$-0.93$&0.07& 3&$-0.41$&    &25&$-1.31$&0.29&0\\
J084424.24+124546&08:44:24.24&+12:45:46.7&2.482&1.8639&$21.00^{+0.10}_{-0.10}$& 1&$-1.54$&0.12& 1&$-1.54$&0.06& 1&$-1.37$&0.12& 1&$-1.66$&0.06&0\\
J075155.10+451619&07:51:55.10&+45:16:19.6&3.341&2.6827&$20.50^{+0.10}_{-0.10}$& 1&$-1.16$&0.13& 1&$-1.16$&0.09& 3&$-0.81$&    & 1&$-1.80$&0.03&32\\
J081813.14+072054&08:18:13.14&+07:20:54.9&4.177&3.2332&$21.15^{+0.10}_{-0.10}$&13&$-1.41$&0.25& 2&$-1.67$&    & 3&$-1.16$&    & 4&$-1.36$&0.07&0\\
J081813.05+263136&08:18:13.05&+26:31:36.9&4.179&3.5629&$20.65^{+0.10}_{-0.10}$&13&$-0.93$&0.24& 2&$-1.17$&    & 3&$-0.68$&    & 4&$-1.10$&0.05&0\\
J081114.32+393633&08:11:14.32&+39:36:33.2&3.073&2.6500&$20.70^{+0.15}_{-0.15}$&13&$-1.44$&0.15&13&$-1.44$&0.15& 3&$-0.67$&    & 1&$-1.70$&0.03&0\\
J132005.97+131015&13:20:05.97&+13:10:15.3&3.352&2.6722&$20.30^{+0.10}_{-0.10}$& 1&$-2.30$&0.10& 1&$-2.30$&0.02& 3&$-0.46$&    & 1&$-2.81$&0.09&0\\

\enddata
\tablenotetext{a}{1=[Si/H]; 2=[Zn/H]; 
4=[S/H] ; 13=Bracked by Si,Zn limits; 14=[Fe/H]+0.3\,dex.}
\tablenotetext{b}{0=No measurement; 1=Si measurement; 2=Si lower limit;
3=Si upper limit; 4=[S/H] ; 5=[O/H] ; 13=S+Si limits}
\tablenotetext{b}{0=No measurement; 1=Zn measurement; 2=Zn lower limit;
3=Zn upper limit}
\tablenotetext{c}{0=No measurement; 1=Fe measurement; 2=Fe lower limit;
3=Fe upper limit; 4=[Ni/H]-0.1dex;
5=[Cr/H] - 0.2dex;
6=[Al/H]; 11-16=Fe, Ni, Cr, Al limits; 25=Mean of Fe limits.}
\tablecomments{Note that none of the limits reported take into account the
uncertainty in the \nhi\ value.}
\tablerefs{
1: \cite{wolfe94};
2: \cite{lu96};
3: \cite{pw96};
4: \cite{pw97b};
5: \cite{lu99};
6: \cite{pw99};
7: \cite{lopez99};
8: \cite{pw00};
9: \cite{petit00};
10: \cite{molaro00};
11: \cite{mirka01};
12: \cite{molaro01};
13: \cite{pro01};
14: \cite{pgw01};
15: \cite{eps+01};
16: \cite{pho+02};
17: \cite{lsp02};
18: \cite{lrd+02};
19: \cite{ldd+02};
20: \cite{lopez03};
21: \cite{songaila02};
22: \cite{p03_esi};
23: \cite{pro03b};
24: \cite{ledoux03};
25: \cite{mirka04};
26: \cite{ledoux06};
27: \cite{akerman05};
28: \cite{obp+06};
29: \cite{shf06};
30: \cite{dz06};
31: \cite{blah};
32: This paper }
 
\end{deluxetable}

